Together Compiler: Continual Compilation for AI Inference

Today's AI workloads are rapidly changing: new models are released more often, model architectures are increasingly diverse, and traffic distributions change frequently. The challenge we face at Together AI is continual optimization for these changing workloads. Compiling a deployment into an optimized forward pass is a challenge that is well-suited for agent hill-climbing. Existing systems struggle with continual compilation due to a tradeoff between measurement throughput and fidelity. Many systems use agents to optimize individual kernels from the inference forward pass using offline benchmarks, but timings are low-fidelity because of data-dependent behavior in primitives like mixture-of-experts (MoE). On the other hand, systems use agents to directly optimize end-to-end engines but suffer from slow engine launch times. To address these challenges, we build Together Compiler (TKCC), the first truly continual agent loop designed for AI inference optimization. To address the throughput-fidelity tradeoff, we propose: (1) a Tiered Persistent Engine that decouples engine launch overheads from forward pass computation; (2) a cost model to select the parallelism configurations that seed the optimization process. We also conduct extensive ablations on agent context management and present our insights on deploying TKCC in production. TKCC outperforms highly-optimized hand-written Megakernels on the Llama 1B workhorse workload by up to 1.7x and the best open source engines on the latest frontier models (Kimi K3, GLM 5.3, MiniMax M3.1 Flash, DeepSeek v4.1 Flash) across hardware platforms by up to 2.6x higher TPS on the InferenceX benchmark. TKCC also sets the state-of-the-art performance at batch size 1, with 1111 TPS on M3.1 Flash and 1205 TPS on DeepSeek v4.1 Flash. Finally, TKCC generalizes beyond frontier language model inference. TKCC serves trillions of tokens across our production fleet.

==> Tables/tab_3_ai_optimizer_gpu_hours.tex <==
\begin{table*}[!t]
\centering\small
\renewcommand{\arraystretch}{1.35}
\begin{tabularx}{\textwidth}{XXXX}
\toprule
System & Resource use & Experiments/GPU-hour & Task \\
\midrule
\rowcolor{blue!10}
\textbf{\shortname{}}
  & \textbf{48 B200-hr}
  & \textbf{$\sim$12.5}
  & Inference Optimization
  \\
  SkyPilot~\cite{kim2026scalingautoresearch}
  & $\sim$128 H100-hr
  & $\sim$7.1 
  & Hyperparameter Search
  \\
  
Modal~\cite{chen2026autoscalingautoresearch}
  & 238 H100-hr
  & 0.5 
  & Hyperparameter Search
  \\
  
Cursor \& NVIDIA~\cite{lin2026multiagentkernels}
  & 13{,}600 B200-hr
  & $\sim$0.3 
  & Kernel Benchmarking
  
  \\
RSI-Inference Bench~\cite{liu2026rsiinference}
  & 48 B200-hr
  & $\sim$0.06 
  & Inference Optimization
  \\

\bottomrule
\end{tabularx}
\vspace{-2pt}
\caption{AI optimizers ranked by experiment throughput. \shortname{} produces $>$200$\times$ more experiments than the next-best OSS system that tackles inference optimization. Others tackle simpler hyperparameter tuning.}
\label{tab:prior-optimizers}
\end{table*}

==> Tables/tab_4_2_throughput_comp.tex <==
\begin{table}[t]
\centering\small
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrr}
\toprule
 & RSI-Inference Bench & \shortname{} \\
\midrule
Experiments          & 1                               & 322 \\

Time per submission & 4.7h & 67 s  \\
Agent idle time                & 76\%                            & 7\% \\
\bottomrule
\end{tabular*}
\vspace{-2pt}
\caption{Experiment throughput comparison.}
\label{tab:exp-tput}
\end{table}

==> Tables/tab_4_3_engine_startup_mlsys.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lr@{}}
\toprule
\multicolumn{2}{@{}l@{}}{\textit{(a) Engine startup, cold boot}} \\
\midrule
Phase & Time (s) \\
\midrule
Process init.               & 69  \\
Model construction          & 71  \\
Weight loading              & 125 \\
KV-cache sizing             & 73  \\
JIT kernel warm-up          & 147 \\
Autotuning                  & 45  \\
API server ready            & 5   \\
CUDA-graph capture, decode  & 34  \\
CUDA-graph capture, prefill & 192 \\
\midrule
\textbf{Total time to serving}   & \textbf{761} \\
\bottomrule
\end{tabular*}

\vspace{1.5em}

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrr@{}}
\toprule
\multicolumn{3}{@{}l@{}}{\textit{(b) The two tiers}} \\
\midrule
Metric & Slow tier & Fast tier \\
\midrule
Layers served              & 60   & 12   \\
Startup to first job (min) & 11   & 3    \\
Hot reload (s)             & 45   & 17   \\
Job time, median (s)       & 64   & 28   \\
Back-to-back var.\ (\%)    & 0.14 & 0.05 \\
Crashes / 1,000 jobs       & 0    & 3.9  \\
\bottomrule
\end{tabular*}
\captionsetup{justification=centering}
\caption{MiniMax-M3.1-Flash on TensorRT-LLM for (a) engine cold startup time (b) slow and fast tiers.}
\label{tab:m31flash}
\end{table}
